Rapid stellar and binary population synthesis with COMPAS

Compact Object Mergers: Population Astrophysics and Statistics (COMPAS; https://compas.science) is a public rapid binary population synthesis code. COMPAS generates populations of isolated stellar binaries under a set of parametrized assumptions in order to allow comparisons against observational data sets, such as those coming from gravitational-wave observations of merging compact remnants. It includes a number of tools for population processing in addition to the core binary evolution components. COMPAS is publicly available via the github repository https://github.com/TeamCOMPAS/COMPAS/, and is designed to allow for flexible modifications as evolutionary models improve. This paper describes the methodology and implementation of COMPAS. It is a living document which will be updated as new features are added to COMPAS; the current document describes COMPAS v02.21.00.

==> sections/excisedtext.tex <==
% \mike{Note to self on where dynamical timescale is used in \COMPAS evolution: (i) HeWD mass transfer mass gain timescale, (ii) used as minimum timestep as long as it 
is greater than 100s, (iii) Printed in CE output}



\section{SSE: Remnants and SNe}

\citet{Hurley:2003ku} provide a modification to this basic Metsel cooling track which better reproduces the detailed models of \citet{Hansen:1999fa}. 


%\subsubsection{Maximum neutron star mass}
%\label{subsubsec:maxium_neutron_star_mass}

Population synthesis codes usually distinguish between neutron stars and black holes by comparing the mass of a compact object against the maximum neutron star mass. The maximum mass of a non-rotating neutron star before it collapses into a \ac{BH} is currently unknown, and represents a key astrophysical quantity of interest. 
This maximum mass, also known as the 
Tolman--Oppenheimer--Volkoff (TOV) limit, depends on the poorly constrained neutron star equation-of-state \citep[see][for a review]{Ozel:2016oaf}. 
Causality and general relativity arguments constrain the maximum neutron star mass to be between 0.1 and 3.0\Msun \citep{RhoadesRuffini:1974PhysRevLett}, while models for the \ac{NS} equation of state reduce this range to 2.2--2.9 \Msun \citep{Kalogera:1996ci}.
The most massive observed pulsars are around 2\Msun \citep{Demorest:2010Nature,Antoniadis:2013pzd,Arzoumanian:2017puf,Cromartie:2019kug}. 
Recent observations of the binary neutron star merger GW170817 have constrained the maximum neutron star mass to $\lesssim2.3$\Msun assuming that the merger product promptly collapsed to a \ac{BH} \citep[][]{Margalit:2017dij, Ruiz:2017due, Shibata:2019ctb, LIGOScientific:2019eut}. 

%\subsubsection{NS/BH radii and luminosities}
%\label{subsubsec:neutron_star_radii}

The exact radii of neutron stars, and the mass-radius relationship are uncertain \citep[for a review see][]{Ozel:2016oaf}. 
Recent observations from the Neutron star Interior Composition Explorer \citep[NICER;][]{Raaijmakers:2019dks,Miller:2019cac,Riley:2019yda}
and through gravitational waves \citep[e.g.][]{Abbott:2018exr,Capano:2019eae} have suggested neutron stars have radii of around 11--12\,km. 
Some evolution of the radius of the \ac{NS} with the mass is expected from theoretical grounds \citep[see e.g.][]{Ozel:2016oaf}. 
However, the largest observed mass of a \ac{NS} has already ruled out most of the equations of state that would lead to a significantly wide (varying of up $\sim 100\%$ within masses of astrophysical interests) range of \ac{NS} radii, and it now seems sensible to assume that most \acp{NS} have similar radii (with variations $\lesssim 10-20\%$).
Considerable variations are however still allowed by a few proposed equations of state \citep[see e.g.][]{Otto:2019zjy} and by the possibility of phase transitions \citep[for a review see][]{Weber:2004kj}.

%\subsubsection{Remant spins}
%\label{subsubsec:remnant_spins}


% lead to electron-capture supernova (ECSN) \citep{1980PASJ...32..303M, 1984ApJ...277..791N,1987ApJ...322..206N, 2008MNRAS.386..553I}, with lower core masses leading to the formation of white dwarfs. 
% \stephen{Floris noticed that, comparing this statement with \S 3.5.1, it is unclear if/how \COMPAS ever forms ONe WDs (since the lower mass limit for that was also stated as 1.6 Msun).}
% \simon{hmm true, yet we do form ONeWDs. Must be a mistake in how it is written.}
% \ilya{[Here is a verbatim quote from Mandel and Mueller, 2020, which describes what \COMPAS really does (and even then oversimplifies -- if you want the full description, look at the code or see \url{https://compashq.slack.com/archives/CM1FDL7L2/p1592188678046500}):]}

% \ilya{We follow the prescription of Hurley et al. (2000) with partial
% amendments from Belczynski et al. (2008) and Fryer et al. (2012)
% to determine which stars undergo electron-capture and regular core collapse
% supernovae. Stars with core masses above 2.25 $M_\odot$ at the
% base of the asymptotic giant branch undergo core-collapse supernovae
% once their carbon-oxygen core reaches the mass threshold of
% equation (75) of Hurley et al. (2000), where we use 1.38 $M_\odot$ in lieu of
% the Chandrasekhar mass. The remnant masses are then computed as
% described above. If the helium core mass is below 2.25 $M_\odot$ but above
% 1.6 $M_\odot$ at the base of the asymptotic giant branch and the mass of the carbon-oxygen core reaches 1.38 $M_\odot$ during subsequent evolution, the star is assumed to form
% an NS with a gravitational mass of 1.26 $M_\odot$ in an electron-capture
% supernova.}


[Mass gap] that is apparent from X-ray binary observations \citep{1998ApJ...499..367B, 2010ApJ...725.1918O, 2011APS..APRH11002F}; a lack of BHs with masses between those of the 
heaviest \acp{NS} $\sim$ 2--3\Msun \citep{2016ARA&A..54..401O, 2017ApJ...850L..19M, 2019NatAs.tmp..439C,2019arXiv190801012T,2020arXiv200106102S} and the lightest BHs of 
$\sim$ 4--7\Msun.  % \citep{2015ApJ...801...90P,2019ApJ...882L..24A}. % However, recent observations of a $\sim2.6$\Msun compact object in the gravitational-wave event 
GW190814 \citep{Abbott:2020khf}, from microlensing \citep{2020A&A...636A..20W} and of $\sim3$\Msun compact objects in Galactic non-interacting binaries 
\citep{2019Sci...366..637T,Jayasinghe:2021uqb} have cast doubt on the existence of a true mass gap.


% Around $\sim 0.1$\Msun is lost from the core of a massive star during the first $\sim 100$\,ms after the core bounce \citep{MandelMueller:2020}. 
% We provide two options for determining the amount of mass lost in neutrinos in BH formation. 
% By default, we simply assume that 10\% of the mass of the collapsing star is lost, following \citet{Fryer:2012ApJ}. 
% However, in reality the amount of mass lost may be much smaller for \acp{BH} if the proto-neutron star collapses to a \ac{BH} after the first $\sim 100$\,ms \citep[see e.g. discussion in ][]{Stevenson:2019rcw,MandelMueller:2020}. 
% As an alternative, we consider a model in which a fixed amount of mass is lost (by default, 0.1\Msun).

% The loss of mass through neutrinos from the center of the star leads to a weak shock propagating out through the star, which may unbind a weakly bound envelope (with a binding energy less than $10^{47}$\,ergs) \citep{Nadezhin:1980,Lovegrove:2013hox,Fernandez:MNRAS}. 
% This may limit the mass of BHs formed from single stars.

% In \COMPAS, we determine remnant masses following the prescription from \citet{Fryer:2012ApJ}. 

% Additional models? \citep{Belczynski:2001uc}.  \citep{Mueller:2016}? 

% \citep{MandelMueller:2020} \citep{Mandel:2020}



% \simon{Figure out where the discussion of remnant mass prescriptions goes amongst the discussion of supernova types.}

%
% From Tauris+ 2015
% Of particular interest for the scenario discussed in this paper is mass transfer by Roche-lobe overflow (RLO) initiated by the helium-star expansion after core helium depletion, i.e. so-called Case BB RLO, first discussed by Savonije & Takens (1976), De Greve & De Loore (1977) and Delgado & Thomas (1981).
% Case BB mass transfer \citep{} from a companion star onto a \ac{NS} or \ac{BH} in short period binaries leads to severe stripping by the compact object (i.e. leaving behind an envelope with mass $\lesssim 0.1$\Msun).



%The existence of a BH mass gap of an absence of BHs with masses in the range $\sim 50$--$150$\Msun is suggested from both observations \citep{2017ApJ...851L..25F,2018ApJ...856..173T,2019PhRvX...9c1040A, 2019PhRvD.100d3012W, 2019MNRAS.484.4216R,2019arXiv191209708G} and theory \citep{1964ApJS....9..201F,1967PhRvL..18..379B,2017ApJ...836..244W, 2019ApJ...887...53F}. \selma{ [1] I'd say theory says the gap may  start as low as 45\Msun, Farmer.  Woosley used non standard nuclear reaction rates. [2] I think the observational evidence so far is only tentative, while the theory prediction has been there for decades. I would change the order. }  
%Stars with helium cores in these mass ranges are thought to become unstable as a result of electron positron pair production. 
%This causes the radiation pressure support in the core to drop, causing the core to contract. 
%As it contracts, the temperature increases, triggering explosive oxygen burning. 
%This may reverse the contraction and completely unbind the star in a pair-instability supernova (PISN) explosion, leaving no remnant behind  \citep{1964ApJS....9..201F,1967PhRvL..18..379B,1968Ap&SS...2...96F,2019ApJ...887...72L,2019ApJ...878...49W,2014A&A...565A..70K,2014A&A...566A.146K,2017MNRAS.464.2854K}.  


% \floor{merge below with above}

% 	 During the supernova event a fraction of the ejected material, $f_{\rm{fb}}$, is assumed to fallback onto the compact object. We use the prescription from Eqs.~16 and 19 in  \citet{Fryer:2012ApJ} to determine this fraction and reduce the natal kick by a factor ($1-f_{\rm{fb}}$) accordingly. This typically reduces the natal kicks of BHs with carbon-oxygen cores above 11\Msun  (for the delayed supernova prescription) to zero. This is in agreement with observations  that show evidence that  BHs might form with lower or no natal kicks although this is still under debate  \citep[][]{1999A&A...352L..87N,2012MNRAS.425.2799R,2013MNRAS.434.1355J,2015MNRAS.453.3341R,2016MNRAS.456..578M}. %,  see also \citealt{2013MNRAS.434.1355J}  and references therein. 
% 	 %
% %	 For ultra-stripped and electron-capture supernova we use instead  a  one-dimensional root-mean-square velocity dispersion of  $\sigma = 30$ \kms  which is in agreement with the subset of double NS / Pulsar systems observed with low velocities and small eccentricities \citep{2017ApJ...846..170T} (Tauris et al. 2017).  
% 	%bimodal SN distribution (e.g., Katz 1975; Arzoumanian et al. 2002).
	
% 	All natal kicks from supernovae are assumed to be isotropic  and we sample the kick polar angles $\theta_k$ and kick azimuthal angles $\phi_k$ from a unit sphere. drawing mean anomalies 
	
%	don't draw a mean anomalies of the orbit are assum at the moment of the supernova event from the range $[0,2\pi]$. \floor{(give ref? I could say: see e.g. dart board??)} \floor{double check the parameter range

%\subsection{Future updates}
%\label{subsec:single_stellar_evolution_future_updates}

% I (Reinhold) removed this section
%The stellar tracks utilised by \COMPAS and many of its contemporaries are from \citet{Pols:1998MNRAS}, as discussed in Section~\ref{sec:single_star}. 
%Whilst these analytical fitting formulae have proven remarkably useful over the years, these tracks have some drawbacks. 
%Firstly, the parameter space for which the original models were calculated is somewhat limited, with a restricted range of metallicities and no stellar models computed above 50\Msun. 
%Secondly, it can be difficult to update these fits to account for improved understanding in massive stellar evolution. 
%We therefore intend in the near future to add the capability to \COMPAS to directly interpolate the properties of stars from a set of detailed stellar tracks \citep[e.g.][]{Eldridge:2016ymr,Kruckow:2018slo,Spera:2018wnw,Agrawal:2020}.% \floor{merge below with above}

% 	 During the supernova event a fraction of the ejected material, $f_{\rm{fb}}$, is assumed to fallback onto the compact object. We use the prescription from Eqs.~16 and 19 in  \citet{Fryer:2012ApJ} to determine this fraction and reduce the natal kick by a factor ($1-f_{\rm{fb}}$) accordingly. This typically reduces the natal kicks of BHs with carbon-oxygen cores above 11\Msun  (for the delayed supernova prescription) to zero. This is in agreement with observations  that show evidence that  BHs might form with lower or no natal kicks although this is still under debate  \citep[][]{1999A&A...352L..87N,2012MNRAS.425.2799R,2013MNRAS.434.1355J,2015MNRAS.453.3341R,2016MNRAS.456..578M}. %,  see also \citealt{2013MNRAS.434.1355J}  and references therein. 
% 	 %
% %	 For ultra-stripped and electron-capture supernova we use instead  a  one-dimensional root-mean-square velocity dispersion of  $\sigma = 30$ \kms  which is in agreement with the subset of double NS / Pulsar systems observed with low velocities and small eccentricities \citep{2017ApJ...846..170T} (Tauris et al. 2017).  
% 	%bimodal SN distribution (e.g., Katz 1975; Arzoumanian et al. 2002).
	
% 	All natal kicks from supernovae are assumed to be isotropic  and we sample the kick polar angles $\theta_k$ and kick azimuthal angles $\phi_k$ from a unit sphere. drawing mean anomalies 
	
%	don't draw a mean anomalies of the orbit are assum at the moment of the supernova event from the range $[0,2\pi]$. \floor{(give ref? I could say: see e.g. dart board??)} \floor{double check the parameter range

%\subsection{Future updates}
%\label{subsec:single_stellar_evolution_future_updates}

% I (Reinhold) removed this section
%The stellar tracks utilised by \COMPAS and many of its contemporaries are from \citet{Pols:1998MNRAS}, as discussed in Section~\ref{sec:single_star}. 
%Whilst these analytical fitting formulae have proven remarkably useful over the years, these tracks have some drawbacks. 
%Firstly, the parameter space for which the original models were calculated is somewhat limited, with a restricted range of metallicities and no stellar models computed above 50\Msun. 
%Secondly, it can be difficult to update these fits to account for improved understanding in massive stellar evolution. 
%We therefore intend in the near future to add the capability to \COMPAS to directly interpolate the properties of stars from a set of detailed stellar tracks \citep[e.g.][]{Eldridge:2016ymr,Kruckow:2018slo,Spera:2018wnw,Agrawal:2020}.


There is evidence from gravitational-wave observations of merging binary \acp{BH} that such a mass gap exists in nature \citep{2017ApJ...851L..25F,2018ApJ...856..173T,2019PhRvX...9c1040A, 2019PhRvD.100d3012W, 2019MNRAS.484.4216R,2019arXiv191209708G}.
[35--45 excess]  has also been suggested from observations \citep{2018ApJ...856..173T,2019PhRvX...9c1040A}. 


The location of the \ac{PISN} gap has been shown to be a robust prediction according to detailed stellar models for naked helium cores (\citealt{2019ApJ...887...53F, Renzo:2020rzx}), although it is somewhat sensitive to uncertain nuclear reaction rates, such as alpha captures onto carbon \citep{Takahashi:2018kkb, 2019ApJ...887...53F, Farmer:2020xne}.
A further uncertainty is whether the H-rich envelope of a star, if still present at the moment of core collapse, can be accreted onto the newly formed \ac{BH} \citep[e.g.][]{2017ApJ...836..244W, Mapelli:2020, Farrell:2020zju, 2020arXiv201002242C}. 
Such considerations are particularly important for the formation of the most massive \acp{BH}, such as those observed in the \ac{BBH} merger GW190521 \citep{Abbott:2020tfl,Abbott:2020mjq}.
In massive close binaries we expect that such an envelope will have been removed due to interaction with the companion.  
We do not expect our particular choice for \ac{PISN} and pulsational-\ac{PISN} prescription to drastically influence our results (see also \citealt{Stevenson:2019rcw}).  


Combined, the pulsar speeds are roughly bimodal, and so the magnitude of supernova kicks can thus be drawn from a bimodal distribution as suggested by \citet{1975Natur.253..698K,2002ApJ...568..289A}.





\section{BSE}

Massive B-type and O-type stars are the progenitors of compact objects \citep[e.g.,][]{Heger2003,Smart:2009ARA&A}.
Observations of massive stars in the field indicate that most of them have at least one stellar companion \citep[e.g.,][]{Sana:2012Sci,Sana:2014,Moe:2017ApJS}.
Stellar multiplicity affects the evolution of the component stars, modifying their properties and creating outcomes impossible for single stars \citep[e.g.,][]{Podsiadlowski:1992ApJ}.
The stellar components of long period binaries can evolve in a similar way to single stars.
On the other hand, the components of close binaries can directly or indirectly interact throughout their lifetimes.


% Finally, in Section \ref{subsec:binary_magnetic_braking} we justify our lack of implementation of magnetic braking.

% \subsection{Tidal interactions}
% \label{subsec:binary_tides}
% \ilya{[Maybe start with what we do, rather than what we do not do?]}
% \avg{[I think a short introduction for someone junior or not in the field is helpful. Moreover because it is only a paragraph.]}
% Close binaries experience tidal interactions \citep[e.g.][]{Zahn:1977A&A,Hut:1981A&A}.
% Tides circularise the orbit and synchronise stellar and orbital spins.
% The evolution and efficiency of tides strongly depend on the configuration of the orbit and the evolutionary stage of a tidally distorted star.
% In rapid population synthesis codes, tidal evolution is usually simplified \citep[see, e.g.,][]{Hurley:2002rf}. 


% In \COMPAS we do not include full tidal evolution. \ilya{[This is the only sentence that should remain in this section; what precedes this is review, and what follows belongs in a section on mass transfer.]}

% We only consider tides at the onset of \ac{RLOF}.
% There are three user-defined possibilities then: the binary remains the same (default), the binary is circularised to periastron, or the binary is cirularised to semi-latus rectum (conserving angular momentum).
% Our default model circularises the binary to periastron.
% For an investigation and discussion on the effects of tides and their uncertainties within the \COMPAS framework see \cite{Vigna-Gomez:2020bgo}.



\citet{2018MNRAS.481.4009V} show that this assumption leads to a better match of population synthesis models to the observed population of  Galactic \ac{DNS} binaries. 


Alternatives to adiabatic mass loss/transfer exponents to determine dynamical stability are critical mass ratios \citep[e.g.,][]{Hurley:2002rf,2014A&A...563A..83C} and 
critical mass transfer rates \citep[e.g.,][]{Pavlovskii:2017MNRAS}.

The details of a mass transfer episode are quite sensitive to the stellar and orbital configuration \citep[see, e.g.,][for a rapid population synthesis analysis]{2015ApJ...805...20S}.
In \COMPAS they depend on the stellar type of the component stars (Section \ref{subsec:evolutionary_stages}) and on the user defined parameterisation of angular momentum loss ($\gamma$ in Equation \ref{eq:mass_transfer_orbital_evolution}).
\avg{
We assume that only stellar components can initiate a mass transfer episode.

We do this numerically by using a ``Bracket and Solve Root" function from the Boost library, with numerical tolerances set in the ``constants.h" file.


		
\begin{equation}
    \dot{M}_{\rm{edd}} = \dfrac{4 \pi G m_{\rm{p}}}{\epsilon c \sigma_{\rm{t}}}M_{\rm{a}},
\end{equation}
where $m_{\rm{p}}$ is the mass of a proton, $\epsilon$ is the fraction of energy released in radiation, and $\sigma_{\rm{t}}$ is the Thomson cross section. 
COMPAS assumes by default an accretion efficiency of  $\epsilon= 0.1$ \citep{2002apa..book.....F}. 


Which of the scenarios more accurately represents observations is still under debate.
Recently, \citet{2017MNRAS.472.2422M} show that the pessimistic scenario matches the predicted BH--BH rate slightly better. 
\citet{2018MNRAS.481.4009V,VignaGomez:2020PASA} argue that there is no clear evidence to favor one of the scenarios over the other based on a study of Galactic NS--NS  binaries.  
\citet{Klencki2020bindingEnergy} uses detailed stellar models to argue that only cool stars with fully convective envelopes and low binding energy can successfully eject their envelope, i.e. that Hertzsprung-gap stars would lead to stellar mergers.

, similar to recent  population synthesis studies including \citet{2018MNRAS.480.2011G,2019ApJ...885....1W,2019MNRAS.490.3740N}.
More details and discussion of the treatment of CEs in {\sc{COMPAS}} are discussed in \citet{VignaGomez:2020PASA} and \citet{2020MNRAS.492.3229H}.



A stellar merger occurs when a star and a stellar or compact object companion merge into a single gravitationally bounded entity.

but the subsequent merger product is evolution is not implemented.
\citet{Hurley:2002rf} has a simple prescription to account for the remnant type of the stellar merger depending on the merging stars (c.f. Table 2 of that paper); the implementation of this prescription is pending.
Currently, there are no robust prescriptions to account for the post-merger properties of these systems.



Many population synthesis codes follow the implementation from \citet{Hurley:2002rf}, which has been found troublesome in the high-mass regime 
\citep[e.g.,][]{Kushnir:2016zee,VignaGomez:2020PASA,2021MNRAS.503.5569V}.



%\subsection{Initial conditions}
%\label{subsubsec:COMPAS_initial_conditions}




%
\begin{align}
%
&\rate_{\rm{form}}(\Zi, \tdelay, \monef, \mtwof) = \notag \\
%
\label{eq:formation-rate-COMPAS}
\end{align}

Making predictions for the occurrence rate of astrophysical events over the history of our Universe is important to understand phenomena such as \acp{SN}, \ac{DCO} mergers and \acp{GRB}, which often can be observed and/or have progenitors out to cosmological distances. 

The  \COMPAS suite provides publicly available python post-processing scripts to calculate cosmological formation and merger rates of astrophysical events. 

The time between the \ac{DCO} formation and merger, i.e. the inspiral time, can span from Myr to many Gyr \citep[e.g.,][]{1994MNRAS.268..871T, 1998A&A...332..173P, 2002ApJ...572..407B,Mapelli:2017hqk}. %%%%%
The \ac{DCO} mergers that are observed today with a ground-based \ac{GW} network, therefore, can originate from progenitors that formed at a wide spread of formation times throughout the history of the Universe, and as a result, a wide range of birth metallicities \Zi. 
Figure~\ref{fig:timescalesEvolution} depicts 
  significant times, and the corresponding evolutionary phases, for the estimation of \ac{DCO} merger rates. 
%%%%

, we therefore first integrate the formation rate from Equation~\ref{eq:formation-rate-COMPAS} over metallicities and use the relation $\tform = \tmerger - \tdelay$ to 
obtain the merger rate for a binary with final masses \monef, \mtwof at any given merger time \tmerger with where \ts is the time in the source frame of the merger and 
\Vc is the co-moving volume, which are obtained using the relationship between source and detector frame from, e.g., \citealt{1999astro.ph..5116H} of $\frac{\diff 
\ts}{\diff \tdet} = \frac{1}{(1+z)}$, where \tdet is the time in the detector frame.


The rate $\rate_{\rm{form}}$ is obtained using the binary evolution simulations of {\sc{COMPAS}} (Section \ref{subsec:method-BPS-merger-rate-per-M-SFR}) and 
${\rm{SFRD}}(\Zi, z(\tform))$\footnote{We use SFRD for the star formation rate density, and \SFRD for the metallicity-specific star formation rate density.} is the 
metallicity-specific star formation rate density, which is a function of birth metallicty \Zi and redshift $z$.

\COMPAS also records important timescales for each system, discussed further in Section~\ref{sec:cosmic_history}.

\COMPAS has the option of producing detailed output, which records important parameters at every time step (see Section \ref{subsec:PostProcessing-recording-Properties}). 

%\footnote{when taking into account the metallicity dependence of the wind velocity at infinity of $v_{\infty} \propto Z^{0.13}$ from \citet{1992ApJ...401..596L}} 

==> sections/formationchannels.tex <==
\section{Formation channels}
\label{sec:formation_channels}

Describe tracking of formation channels, give examples


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/updates.tex <==



\subsection{april 17 -23 2020 -- FSB}
Restructured main.tex: moved sections into separate .tex files that are imported in main.tex
filled in a big part of the introduction 
added several references to introduction 
added \acp{}, and tried to make this consistent throughout text  
made the units notation consistent (e.g. \Msun) 
merged subsections where not yet merged between Simon's and mine text
added section on general \COMPAS before SSE and BSE 
moved sampling to general \COMPAS 
moved post-processing to one section 
added new section on results. I think this will be the demos. 
merged winds in SSE section 
filled in paragraphs on initial distribution functions
merged SN parts
added sections in BSE and filled in most of them. 
Added GW timescale section 
made first attempt figure on different remnant presciptions
added figures on demos. (first attempt) 
merged Appendices 
added PostProcessing sections :-) 
added Appendix B, C and D

%%%%%%%%%%%%%%
